Selective information exchange in collaborative clustering using regularized Optimal Transport

Collaborative learning has recently achieved very significant results. It still suffers, however, from several issues, including the type of information that needs to be exchanged, the criteria for stopping and how to choose the right collaborators. We aim in this paper to improve the quality of the collaboration and to resolve these issues via a novel approach inspired by Optimal Transport theory. More specifically, the objective function for the exchange of information is based on the Wasserstein distance, with a bidirectional transport of information between collaborators. This formulation allows to learns a stopping criterion and provide a criterion to choose the best collaborators. Extensive experiments are conducted on multiple data-sets to evaluate the proposed approach.

==> summary.tex <==
%\renewcommand*{\arraystretch}{1.2}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\setlength\LTleft{0pt}
\setlength\LTright{0pt}
\begin{longtable}{@{\extracolsep{\fill}}>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c}
\caption{A summary of contributions presented in this survey for learning bounds in domain adaptation. \textbf{(Task)} refers to the considered learning problem; \textbf{(Framework)} specifies the statistical learning framework used in the analysis; \textbf{(Divergence)} is the metric used to compare the source and target distributions; \textbf{(Link)} stands for the dependence between the source error and the divergence term; \textbf{(Non-estim.)} indicates the presence of a non-estimable term in the bounds.} 
\endfirsthead
\endhead
\toprule
\addlinespace[.1cm]
\multirow{3}{*}{\footnotesize{\textbf{\textsc{Reference}}}}& \multicolumn{5}{c}{\footnotesize{\textbf{\textsc{Learning bounds}}}}\\
\addlinespace[.1cm]\cline{2-6}
\addlinespace[.1cm]
& \textbf{\textsc{Task}} & \textbf{\textsc{Framework}} & \textbf{\textsc{Divergence}} &	\textbf{\textsc{Link}} & \textbf{\textsc{Non-estim.}}\\
\addlinespace[.1cm]
\toprule
\addlinespace[.1cm]
\makecell{\cite{BenDavid07analysisof}\\\cite{Blitzer07Learning}\\\cite{bendavidth}} & \makecell{Binary\\ classification} & VC & $L^1$, $\hdh$ & Add. & $+$\\
\hline
\addlinespace[.1cm]
\cite{MansourMR09colt} & \makecell{Classification/\\ Regression} & Rademacher & Discrepancy & Add. & $+$\\
\addlinespace[.1cm]
\hline
\makecell{\cite{CortesMM10}\\\cite{CortesM14}\\\cite{CortesMM15}} & Regression & Rademacher & \makecell{(Generalized)\\ Discrepancy} & Add. & $+$\\
\hline
\addlinespace[.1cm]
\cite{KurokiCBHSS19} & \makecell{Classification} & Rademacher & (S-)Discrepancy & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{MansourMR08multiple} & \makecell{Classification/\\ Regression} & -- & -- & -- & --
\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\makecell{\cite{MansourMR09}\\\cite{HoffmanMZ18}} & \makecell{Classification/\\ Regression} & -- & R\'enyi & Mult. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{DhouibR18} & \makecell{Binary classification/\\Similarity learning} & -- & $L^1$, $\chi^2$ & Mult. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{RedkoCFT19} & Binary classification & Rademacher & Discrepancy & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{ZhangZY12} & \makecell{Regression/ \\ Classification} & \makecell{Uniform \\entropy number} & IPM & Add. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{Redko15} & Regression & Rademacher & IPM/MMD & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{RedkoHS16} & Regression & -- & IPM/Wassertein & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{zhang_bridging_2019} & \makecell{Large-margin\\classification} & Rademacher & IPM & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{JohanssonSR19} & \makecell{Classification} & -- & IPM & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{ShenQZY18} & Classification & -- & Wasserstein & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{CourtyFHR17} & Classification & -- & Wasserstein & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{pbda} & \makecell{Classification} & PAC-Bayes & Domain disagreement & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{dalc} & \makecell{Classification} & PAC-Bayes & $\beta$-divergence & Mult. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{li2007bayesian} & Classification & PAC-Bayes & -- & Add. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{McNamaraB17} & \makecell{Binary classification} & VC/PAC-Bayes & -- & Add. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{MansourS14} & Classification & Robustness & $\lambda$-shift & Add. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.05cm]
\makecell{\cite{KuzborskijO13}\\\cite{KuzborskijO17}\\\cite{simonHTL}} & Regression & Stability & -- & -- & --\\
\addlinespace[.05cm]
\hline
\addlinespace[.1cm]
\cite{PerrotH15ICML} & \makecell{Classification/\\Similarity learning} & Stability & -- & -- & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{MorvantKAIS12} & \makecell{Classification/\\Similarity learning} & Robustness/VC & $\hdh$ & Add. & +\\
\addlinespace[.1cm]
\bottomrule
\end{longtable}
\begin{longtable}{@{\extracolsep{\fill}}>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c}
\caption{A summary of contributions presented in this survey for hardness results in domain adaptation. \textbf{(Type)} is the type of the obtained result; \textbf{(Setting)} points out the presence or absence of target data (either labelled or unlabelled); \textbf{(Assumptions)} indicate the considered assumptions (individual or combined); \textbf{(Proper)} specifies if the learned model is required to belong to a predefined class; \textbf{(Constr.)} indicates if the result is of a constructive nature.} 
\endfirsthead
\endhead
\toprule
\addlinespace[.1cm]
\multirow{3}{*}{\footnotesize{\textbf{\textsc{Reference}}}}& \multicolumn{5}{c}{\footnotesize{\textbf{\textsc{Hardness results}}}}\\
\addlinespace[.1cm]\cline{2-6}
\addlinespace[.1cm]
& \textbf{\textsc{Type}} & \textbf{\textsc{Setting}} & \textbf{\textsc{Assumptions}} &	\textbf{\textsc{Proper}} & \textbf{\textsc{Constr.}}\\
\addlinespace[.1cm]
\toprule
\addlinespace[.1cm]
\cite{BenDavidLLP10} & \makecell{Impossibility/\\Sample compl.} & Unlabelled target & \makecell{Cov. shift,\\$\hdh$, $\lambda_\Hcal$} & -- & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{BenDavidSU12} & \makecell{Impossibility/\\Sample compl.} & \makecell{No target/\\Unlabelled target} & \makecell{Cov. shift,\\$C_{\cal B}$, Lipscht.} & $+$ & $+$/--\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{BenDavidU12} & \makecell{Impossibility/\\Sample compl.} & \makecell{Unlabelled target} & \makecell{Cov. shift,\\$C_{\cal B}$, Realizab.} & -- & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{RedkoHS19} & \makecell{Estimation/\\Sample compl.} & \makecell{Labelled target} & -- & -- & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{CZG19} & \makecell{Impossibility} & \makecell{Unlabelled target} & \makecell{Cov. shift,\\$\hdh$, $\lambda_\Hcal$} & -- & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{JohanssonSR19} & \makecell{Impossibility} & \makecell{Unlabelled target} & \makecell{Cov. shift,\\$\hdh$, $\lambda_\Hcal$} & -- & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{hanneke19} & \makecell{Sample compl.} & \makecell{Labelled target} & \makecell{Relaxed cov. shift,\\Noise cond.} & -- & --\\
\bottomrule
\end{longtable}
%
